Multilingual Fact Linking

Knowledge-intensive NLP tasks can benefit from linking natural language text with facts from a Knowledge Graph (KG). Although facts themselves are language-agnostic, the fact labels (i.e., language-specific representation of the fact) in the KG are often present only in a few languages. This makes it challenging to link KG facts to sentences in languages other than the limited set of languages. To address this problem, we introduce the task of Multilingual Fact Linking (MFL) where the goal is to link fact expressed in a sentence to corresponding fact in the KG, even when the fact label in the KG is not available in the language of the sentence. To facilitate research in this area, we present a new evaluation dataset, IndicLink. This dataset contains 11,293 linked WikiData facts and 6,429 sentences spanning English and six Indian languages. We propose a Retrieval+Generation model, ReFCoG, that can scale to millions of KG facts by combining Dual Encoder based retrieval with a Seq2Seq based generation model which is constrained to output only valid KG facts. ReFCoG outperforms standard Retrieval+Re-ranking models by 10.7 pts in Precision@1. In spite of this gain, the model achieves an overall score of 52.1, showing ample scope for improvement in the task.ReFCoG code and IndicLink data are available at https://github.com/SaiKeshav/mfl

==> sections/error_analysis.tex <==
% We check the errors associated with 100 valdiation examples and find the following trend:
% We discover the following types of errors in 100 validation examples with incorrect predictions: 
We analyze the errors made by \shortn{} and classify it into the following three types:
\begin{enumerate*}[label=(\arabic*)]
    \item \textbf{Rare relations}: The model fails to output facts that contain rare relations. This can be traced back to the WebRED training data where the top-10 relations are responsible for 80\% of the examples.
    \item \textbf{\textsc{Null} fact}: The model wrongly predicts \textsc{Null} in 33\% of the examples, demonstrating the difficulty in detecting absence of any facts.
    \item \textbf{Issues with Gold}: 
    % Few sentences refer to entities that can be extracted only after running coreference resolution on the paragraph from which it is taken.
    Few examples contain relations that are not explicitly implied by the sentence but require background world knowledge.
\end{enumerate*}   

% \begin{itemize}
%     \item \textbf{Rare relations}: The model struggles to output facts that contain rare relations. This can be traced back to the WebRED training data where 90\% facts contain top-10 relations.    
%     \vspace{-1ex}
%     \item \textbf{\textsc{Null} fact}: Model wrongly predicts \textsc{Null} in xx\% of the examples, demonstrating the difficulty in linking to \textsc{Null} facts.
%     \vspace{-1ex}
%     \item \textbf{Issues with Gold}: There are some mistakes in gold annotation of Wikidata entities and relations. 
%     \vspace{-1ex}
% \end{itemize}

% We show qualitative predictions of the \shortn{} model in \Cref{app:qualitative_examples}. 
